Unveiling process insights from refactoring practices

Context : Software comprehension and maintenance activities, such as refactoring, are said to be negatively impacted by software complexity. The methods used to measure software product and processes complexity have been thoroughly debated in the literature. However, the discernment about the possible links between these two dimensions, particularly on the benefits of using the process perspective, has a long journey ahead. Objective: To improve the understanding of the liaison of developers' activities and software complexity within a refactoring task, namely by evaluating if process metrics gathered from the IDE, using process mining methods and tools, are suitable to accurately classify different refactoring practices and the resulting software complexity. Method: We mined source code metrics from a software product after a quality improvement task was given in parallel to (117) software developers, organized in (71) teams. Simultaneously, we collected events from their IDE work sessions (320) and used process mining to model their processes and extract the correspondent metrics. Results: Most teams using a plugin for refactoring (JDeodorant) reduced software complexity more effectively and with simpler processes than the ones that performed refactoring using only Eclipse native features. We were able to find moderate correlations (43%) between software cyclomatic complexity and process cyclomatic complexity. The best models found for the refactoring method and cyclomatic complexity level predictions, had an accuracy of 92.95% and 94.36%, respectively. Conclusions: Our approach agnostic to programming languages, geographic location, or development practices. Initial findings are encouraging, and lead us to suggest practitioners may use our method in other development tasks, such as, defect analysis and unit or integration tests.

==> RQ5.tex <==
\subsection{\textbf{RQ4. Can we discover patterns of development in manual refactoring tasks?.}}
Teams doing automatic refactoring used the \textit{JDeodorant} plugin to detect refactoring opportunities and fix them. That set of teams do not provide rich information about the activities developers do, since the plugin does all the heavy workload in the refactoring. As such, we used only the subset of teams doing manual refactoring to discover coding patterns within their activities. 

Figure \ref{chapter7-2.pdf} provides an small sample of the activities/commands issued by developers. Word sizing represent the probability of that word belong to a specific topic. The bigger the word the higher the probability it has to fit into that pattern.  From these, we computed the optimal number of patterns(topics) assessing the probabilistic coherence of topics. This measurement approximates semantic coherence or understandability of a topic, and we used it to decide the final number of patterns to use in training models ranging the number (\textit{\textbf{k}}), from 1 to 10.

\plot{chapter7-2.pdf}[A sample of a team work session frequent actions/commands][12][H][trim=6cm 9cm 4cm 9cm]

Figure \ref{chapter9-1.pdf} shows the coherence values for all models. As seen, 2 was the optimal value found. Figure \ref{chapter7-1.pdf} render the terms for the two patterns.

\plot{chapter9-1.pdf}[Optimal number of patterns(topics) to mine][12][H][trim=0cm 0cm 0cm 0cm]

\textbf{Observation X.1: Pattern identified as 1, denotes a refactoring practice mainly based only on individual skills and/or using a third-party tool.} As one can easily see, it groups teams which have done often navigation(File Open, Close, Save), regular editing (Editing, Copy, Paste, Delete) and refactoring opportunity detection, such as Good Class, Long Method, Type Checking and Feature Envy. However, we don't find in the top terms, with relevant \textit{Beta} values, the presence of any refactor activity or command.

\textbf{Observation X.2: Pattern 2 show evidences for a practice supported by the IDE native features.} In addition to the trivial Editing and refactoring opportunity detection commands, we find reference to Extract Method, Extract Class and Move activities. Table \ref{table:topics-patterns} lists the top 15 teams and their correspondent metrics for \textbf{VG} and \textbf{PCC}, in descent order by software complexity reduction(\textbf{VG}), together with the topic(labelled accordingly) to which they were associated. Each team was assessed in this exercise, in terms of the code smells detected and their correction. Metric \textbf{GRADE} refers to the mark each team had, where higher values mean better performance.

\textbf{Observation X.3: Pattern 2 teams excel in relevant metrics.} The median grade for teams in pattern 1 was 2.065, in pattern 2 was 2.5. 
Pattern 1 teams had 550.5 as median in process cyclomatic complexity, whereas pattern 2 had 331.
Software complexity had a median reduction of 4.52\% for teams in pattern 1, 4.75\% for pattern 2.
As one can quickly discover, teams grouped as pattern 2, which we labelled in Table \ref{table:topics-patterns} as using Eclipse Native Features, had better performance in all the evaluated perspectives.

\plot{chapter7-1.pdf}[Development patterns found][12][H][trim=0cm 0cm 0cm 0cm]

We have however a non-expected finding in the results, the case of team \textbf{A}. This team had the highest reduction in software cyclomatic complexity apparently without using any IDE refactoring functionality or simply using them very infrequently. We conducted a detailed investigation on this team and we came across some interesting insights. 

\textbf{Observation X.4: Team A are experienced developers with very good skills or they simply used an external tool to refactor their code.}
Team A reduced the average lines of code per method (\textbf{MLOC}) in $\approx$15.75\%, and the number of methods \textbf{NOM} in $\approx$6.9\%, however, they increased the total lines of code \textbf{TLOC} by $\approx$5.48\%. Further investigation revealed they increased the average number of classes per package fragment \textbf{NOC} by $\approx$34\%. We don't have any evidence that this was achieved using the Eclipse functionalities, therefore, we cannot exclude the possibility that team A used any other external tool to refactor their code. Even if that was the case, we would signal this code as candidate for deeper bug detection since a unknown practice was used to refactor.




\input{topics-patterns}

\input{pseudo-code}



==> accuracy_matrix.tex <==
\begin{table}[H]
\caption{Accuracy Matrix}
\label{table:accuracy-matrix}
%\centering
\begin{tabular}{ccccccccc}
	\hline\noalign{\smallskip}
			\textbf{Model} & \textbf{TP} & \textbf{FP} & \textbf{Precision} & \textbf{Recall} & \textbf{F-Measure} & \textbf{MCC} & \textbf{ROC} & \textbf{PRC}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
	%\multicolumn{8}{l}{\textbf{Automatic Refactoring}}\\[0.1cm]
     
     \textbf{M1*} & 0.625 &   0.083 & 0.714 & \textbf{0.625} & 0.667 & 0.567 & 0.776 & 0.726\\[0.1cm]
     \textbf{M2} & 0.875 &   0.250  &  0.538 & 0.875 & 0.667 & 0.551 & \textbf{0.870} & 0.716\\[0.1cm]
     
    % \input{chapter7-topics_latex}
     
   \noalign{\smallskip}\hline
   \multicolumn{9}{l}{\textbf{TP}-True Positive, \textbf{FP}-False Positive, \textbf{MCC}-Matthews Correlation Coefficient}\\
    \multicolumn{9}{l}{\textbf{ROC}-Receiver Operating Characteristic, \textbf{PRC}-Precision-Recall Curve}
   %\multicolumn{4}{l}{\shortstack[l]{\textbf{Df.} - Degrees of freedom, \textbf{Chi-Sq.} - Chi-Square,\\ \textbf{Sig.} - Asymptotic Significance (2-tailed)}}
\end{tabular}
\end{table}

==> anova.tex <==
\begin{table}[H]
\caption{One-Way ANOVA Results}
\label{table:aov}
%\centering
\begin{tabular}{clccccc}
	\hline\noalign{\smallskip}
	\textbf{Task} & \textbf{Factor} & \textbf{Df.} & \textbf{Sum Sq.} & \textbf{Mean Sq.} & \textbf{F-value} & \textbf{\textit{p-value}}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
	%\multicolumn{8}{l}{\textbf{Automatic Refactoring}}\\[0.1cm]
     \textbf{\multirow{2}{*}{\shortstack[c]{Automatic\\ Refactoring}}} & \textbf{IV} & 2 & 288 & 2345 &  10 & \textbf{0.0312*}\\[0.05cm] 
     & \textbf{Residuals} &  & 288 & 2345 &  10 & \textbf{0.0312*}\\\\[0.05cm] 
  
     \textbf{\multirow{2}{*}{\shortstack[c]{Manual\\ Refactoring}}} & \textbf{IV} & 2 & 288 & 2345 &  10 & \textbf{0.0312*}\\[0.05cm] 
     & \textbf{Residuals} &  & 288 & 2345 &  10 & \textbf{0.0312*}\\[0.02cm] 
     \noalign{\smallskip}\hline
   \multicolumn{7}{l}{\textit{*Statistically significant if p-value $<$ 0.05}}\\
   \multicolumn{7}{l}{\shortstack[l]{\textbf{Df.} - Degrees of freedom, \textbf{Sum Sq.} - Sum of Square, \textbf{Mean Sq.} - Mean of Square}}
\end{tabular}
\end{table}

==> chapter7-ComplianceDataset.tex <==
%tvaoa1-M & 26B 
A & 2.25 & 518 & 13.981\% & 1 - Manual Skills\\[0.1cm]
%emmms1-M & 11A 
B & 2.42 & 105 & 10.094\% & 2 - Eclipse Native Features\\[0.1cm]
%pggco-M & 24A
C & 1.83 & 554 & 9.528\% & 2 - Eclipse Native Features\\[0.1cm]
%fdtmg-M & 17A 
D & 2.5 & 337 & 7.811\% & 2 - Eclipse Native Features\\[0.1cm]
%fpaos-M & 22B
E & 2.5 & 499 & 6.207\% & 2 - Eclipse Native Features\\[0.1cm]
%lmmfs-M & 13A
F & 2.5 & 219 & 5.792\% & 2 - Eclipse Native Features\\[0.1cm]
%fdcds-M & 14A 
G & 0.17 & 152 & 4.754\% & 2 - Eclipse Native Features\\[0.1cm]
%jmbmo1-M & 23A
H & 1.88 & 583 & 4.528\% & 1 - Manual Skills\\[0.1cm]
%nmglf-M & 14B
K & 2.5 & 464 & 4.528\% & 1 - Manual Skills\\[0.1cm]
%rfcms-M & 21B
L & 2.5 & 201 & 4.245\% & 2 - Eclipse Native Features\\[0.1cm]
%dffrs-M & 19A
M & 1.29 & 738 & 3.603\% & 1 - Manual Skills\\[0.1cm]
%jdsfa1-M & 15A
N & 2.5 & 331 & 3.075\% & 2 - Eclipse Native Features\\[0.1cm]
%mspor-M & 4B
O & 2.5 & 488 & 2.471\% & 2 - Eclipse Native Features\\[0.1cm]
%mcsss-M & 11B
P & 2.5 & 104 & 2.169\% & 2 - Eclipse Native Features\\[0.1cm]
%agfca-M & 26A
Q & 2.25 & 625 & 1.566\% & 2 - Eclipse Native Features\\[0.2cm]

%eptaa-M & 21A & 2.42 & 128 & 1.56603773584906 & 1
%mrpos-M & 7 & 2.44 & 364 & 1.56603773584906 & 1
%barco-M & 18A & 2.42 & 376 & 1.26415094339623 & 1
%bipoa-M & 5B & 1 & 202 & 1.22641509433961 & 2
%acpla-M & 1A & 2.5 & 131 & 0.943396226415091 & 2
%bjfna-M & 6A & 2.5 & 543 & 0.943396226415091 & 2
%cacaa-M & 4A & 2.5 & 222 & 0.943396226415091 & 2
%cpfaa11-M & 3A & 2.5 & 305 & 0.943396226415091 & 2
%gacos-M & 6B & 2.5 & 275 & 0.943396226415091 & 2
%jmgas1-M & 8B & 2.5 & 314 & 0.943396226415091 & 2
%jpmna-M & 17B & 2.5 & 183 & 0.943396226415091 & 2
%mccta-M & 9A & 2.25 & 270 & 0.943396226415091 & 2
%reavh-M & 13B & 2.5 & 436 & 0.943396226415091 & 2
%absta-M & 51 & 2.38 & 296 & 0.622641509433952 & 1
%ajcvo-M & 22A & 2.5 & 196 & 0.622641509433952 & 1
%fcfaa-M & 2A & 2.25 & 93 & 0.622641509433952 & 2
%fmmcp-M & 3B & 2.5 & 242 & 0.622641509433952 & 2
%jmmpa111-M & 16A & 2.5 & 53 & 0.622641509433952 & 1
%jtaca-M & 10A & 2.5 & 85 & 0.622641509433952 & 2
%opmna-M & 16B & 2.5 & 130 & 0.622641509433952 & 2
%rmsca111-M & 10B & 2.5 & 306 & 0.622641509433952 & 2
%trgsb-M & 23B & 2.33 & 378 & 0.622641509433952 & 1
%afcma11-M & 31A & 2.42 & 152 & 0.320754716981122 & 2
%mpcts-M & 29A & 2.5 & 114 & 0.320754716981122 & 1


==> chapter7-topics_latex.tex <==
\multirow{10}{*}{1} & Editing & Eclipse Editor-File Editing & 0.257\\[0.2cm]
& Navigation & Eclipse View-Package Explorer & 0.213\\[0.2cm]
& Editing & Eclipse Editor-File Open & 0.107\\[0.2cm]
& Refactoring & Eclipse View-God Class & 0.107\\[0.2cm]
& Editing & Eclipse Editor-File Close & 0.093\\[0.2cm]
& Refactoring & Eclipse View-Feature Envy & 0.077\\[0.2cm]
& Refactoring & Eclipse View-Long Method & 0.038\\[0.2cm]
& Refactoring & Eclipse View-Type Checking & 0.035\\[0.2cm]
\hline\\
\multirow{10}{*}{2} & Editing & Eclipse Editor-File Editing & 0.400\\[0.2cm]
 & Refactoring & Eclipse View-Long Method & 0.272\\[0.2cm]
 & Refactoring & Eclipse View-Feature Envy & 0.084\\[0.2cm]
 & Refactoring & Eclipse View-God Class & 0.067\\[0.2cm]
 & Editing & Eclipse Editor-File Open & 0.034\\[0.2cm]
 & Editing & Eclipse Editor-File Close & 0.021\\[0.2cm]
 & Navigation & Eclipse View-Project Explorer & 0.020\\[0.2cm]
 & Refactoring & Eclipse View-Type Checking & 0.019\\[0.2cm]
\hline\\
\multirow{10}{*}{3} & Editing & Eclipse Editor-File Editing & 0.272\\[0.2cm]
 & Editing & Edit-Undo & 0.223\\[0.2cm]
 & Navigation & File-Save & 0.093\\[0.2cm]
 & Editing & Eclipse Editor-File Open & 0.072\\[0.2cm]
 & Refactoring & Eclipse View-Long Method & 0.058\\[0.2cm]
 & Editing & Eclipse Editor-File Close & 0.057\\[0.2cm]
 & Editing & Edit-Paste & 0.041\\[0.2cm]
 & Editing & Edit-Delete & 0.027\\[0.2cm]


==> correlation2.tex <==
\begin{table}[H]
\caption{Pearson Correlation}
\label{table:pearson-correlation}
\centering
\begin{tabular}{lcc}
	\hline\noalign{\smallskip}
	\textbf{Factors} & \textbf{Pearson's r} & \textbf{p-value}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

 \input{correlation1_body}

   \noalign{\smallskip}\hline
\end{tabular}
\end{table}

==> correlation3.tex <==
\begin{table}[H]
\caption{Kendall Correlation}
\label{table:kendall-correlation}
\centering
\begin{tabular}{lcc}
	\hline\noalign{\smallskip}
	\textbf{Factors} & \textbf{Kendall's tau} & \textbf{p-value}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

 \input{correlation1_body}

   \noalign{\smallskip}\hline
\end{tabular}
\end{table}

==> correlation_man.tex <==

\begin{table}[H]
\caption{Spearmans' Correlation - Manual Refactoring}
\label{table:spearman-manual-correlation}
%\centering
\begin{tabular}{lcc}
	\hline\noalign{\smallskip}
	& \multicolumn{2}{c}{\cellcolor{gray!10}\textbf{VG}}\\
	\textbf{Factors} & \textbf{\textit{Spearmans' rho}} & \textbf{\textit{p-value}}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

 \input{correlation_man_body}

   \noalign{\smallskip}\hline
   	\multicolumn{3}{l}{\textit{*Statistically significant if p-value $<$ 0.05}}
\end{tabular}
\end{table}


==> correlation_man_body.tex <==
\textbf{PCC} & \textbf{0.43} & \textbf{0.0432*}\\[0.2cm]
\textbf{UF} & 0.32 & 0.3427\\[0.2cm]
\textbf{SES} & 0.24 & 0.2814\\[0.2cm]
\textbf{DEV} & 0.03 & 0.8193\\[0.2cm]
\textbf{NPER} & \textbf{0.32} & \textbf{0.0197*}\\[0.2cm]
\textbf{NISP} & \textbf{0.35} & \textbf{0.0120*}\\[0.2cm]
\textbf{PCCPF} & \textbf{0.45} & \textbf{0.0059*}\\[0.2cm]
\textbf{NCAT} & \textbf{0.39} & \textbf{0.0096*}\\[0.2cm]
\textbf{NCOM} & 0.42 & 0.0712\\[0.2cm]



==> experiment2.tex <==

\subsection{\textbf{RQ3. Are there significant differences in productivity due to the development process?.}}

Automatic
IV - PCC\_LEVEL\\
DV - Productivity\\
DV - KS not normal, SW not normal\\
KW - There are differences\\

Manual
Manual
IV - PCC\_LEVEL\\
DV - Productivity\\
DV - KS not normal, SW not normal\\
KW - There are no differences\\


Removing Outliers\\
Automatic
IV - PCC\_LEVEL\\
DV - Productivity\\
DV - KS Is normal, SW Is normal\\
ANOVA - There are differences\\

Manual
IV - PCC\_LEVEL\\
DV - Productivity\\
DV - KS Is normal, SW Not normal\\
KW - There are no differences\\

\input{variables}

\input{normality}
%\input{variance}
\input{anova}
\input{kruskal-wallis}




In the context of process, methodologies and productivity, existing concepts need to be redefined for meeting the
current needs of the industry. Software process is a well-investigated research area, but nowadays there are several
new advancements in technology and practice that introduce significant changes in this aspect. A new notion of
productivity should be defined, where “lines of code” is not anymore the right measure of productivity, but software
is measured in terms of its other qualities, usability, reliability, scalability \cite{Casale2016CurrentApplications}.

New possibilities to easily gather user
feedback and monitoring information have the potential to enable an informed evolution of software while shorter
development cycles call for novel software production methodologies to actually enable controlled management of
such short development cycles. 

Automatic and manual refactoring tasks had very different results on code cyclomatic complexity reduction and on process cyclomatic complexity. The magnitude of these differences imply that we may not be able to compare productivity between groups accurately only with the initial metrics. Therefore, we decided to compute a new metric to represent teams' productivity.

We computed productivity as follows: 
\begin{equation}
\label{equ:Productivity}
\shortstack[l]{Productivity} =  \frac{Software\ Complexity\ Reduction(\%)}{Work\ Complexity} = \frac{VG}{PCC}
\end{equation}


This new metric allowed us to have a standard way to compare the work done by groups of teams which had completely different conditions to perform the task.

The new metric, resulting from Equation \ref{equ:Productivity}, was analyzed 

To test the hypothesis of normality we have applied the Kolmogorov-Smirnov one-sample test, which is based on the maximum difference between the sample cumulative distribution and the hypothesized cumulative distribution. The underlying hypotheses for this test are the following:
Even considering a confidence interval of 99\% (which is the same to say that $\alpha = 0.01$ and the probability of \textbf{Type I} error of 1\%) we can conclude, from Table 26, that we must reject the null hypothesis for all variables, since we get a significance p $<$ $\alpha$, which means that we have significant Z statistics for all variables being analyzed. In other words, we cannot sustain that the considered variables of our sample come from a Normal population. As such, we can only use non-parametric tests in this experiment.

Regarding the forth assumption, we tested the normality using two well-known tests of normality, namely the Kolmogorov-Smirnov Test and the Shapiro-Wilk test. We will only consider the results of the Shapiro-Wilk test to assess normality since the latter is more appropriate for small sample sizes ($<$ 50 samples).


Due to the fact that those schedules are not normally distributed, we can only perform a non-parametric analysis of variance. We will use the Kruskal-Wallis one-way analysis of variance, an extension of the Mann-Whitney U test, which is the non- parametric analog of one-way ANOVA test. The Kruskal-Wallis H test allows assessing whether several independent samples are drawn from the same population (i.e. if they have similar statistical distributions). In our case those independent samples are the groups of incidents for each of the four Impact valid values.

Let T be a schedule and i and j two different impact categories. Then, the underlying hypotheses for this test are the following:

%\begin{equation}
%\label{equ:diff-tests}
\begin{center}

\hypnull: $\forall$\textsubscript{i,j} : T\textsubscript{i} $\sim$ T\textsubscript{j} \hspace{1cm} vs. \hspace{1cm} \hypalt : $\neg$ $\forall$\textsubscript{i,j} : T\textsubscript{i} $\sim$ T\textsubscript{j}

\end{center}

%\end{equation}

\input{teams-productivity}

We applied the outlier reduction and remain with a dataset of 63 teams. On each susbset, automatic and manual, 4 teams were removed due to be outliers.

\plot{chapter4-9.pdf}[Productivity Index][12][H][trim=0cm 0cm 0cm 0cm]

From Figure \ref{chapter4-9.pdf} one can easily observe that teams performing automatic refactoring were able to obtain in general, higher productivity rates, than the ones using manual refactoring.
We can initially think that the more refactoring activities a team executes, the more productive they may become, or at least they can stabilize within certain productivity levels. That is not confirmed in the automatic refactoring task, as shown by Figure \ref{chapter4-9.pdf}, which reveals that teams with high productivity levels, were the ones with \textbf{LOW} and \textbf{MEDIUM} complexity processes, with very few exceptions. On the other side, we confirm that the less productive teams were the ones where the process complexity levels were \textbf{HIGH} and \textbf{VERY HIGH}. This leads us to think that there is an \textit{equilibrium moment}, which when crossed does make the productivity to reduce substantially. There are some evidences to sustain that, more activities in the IDE did not contribute to the reduction in the product cyclomatic complexity.

We did not find the same pattern in those teams performing manual refactoring. Productivity does not have the same distribution, nor the processes followed by the teams had the same outcomes. There were some teams more productive than others doing automatic refactoring, however, that number is reduced. Teams doing manual refactoring, not only produced less reduction the product cyclomatic complexity, they also were less productive, as they had to work more in the IDE to get the same reductions as the automatic refactoring teams had. In this subset, the process complexity does not seem to linked with the productivity.


We assessed if there are any significant differences between the complexity reduction obtained and the teams having different process complexity levels, which we grouped previously as \textbf{LOW, MEDIUM, HIGH, VERY HIGH}.


\noteboard{RQ3. Summary}{
i) A moderate correlation \textbf{(0.43)} was found between \textbf{VG} and \textbf{PCC} on \textbf{MR} tasks\\
ii) 
}




\noindent\subsection{\textbf{RQ4. Does the development process impact the size of software?.}}


Automatic
IV - PCC\_LEVEL\\
DV - TLOC\\
DV - KS Is normal, SW Is normal\\
ANOVA - There are no differences\\

Manual
Manual
IV - PCC\_LEVEL\\
DV - TLOC\\
DV - KS not normal, SW not normal\\
KW - There are no differences\\


Removing Outliers\\
Automatic
IV - PCC\_LEVEL\\
DV - TLOC\\
DV - KS Is normal, SW Is normal\\
ANOVA - There are no differences\\

Manual
IV - PCC\_LEVEL\\
DV - TLOC\\
DV - KS not normal, SW Not normal\\
KW - There are no differences\\


\noteboard{RQ4. Summary}{
i) A moderate correlation \textbf{(0.43)} was found between \textbf{VG} and \textbf{PCC} on \textbf{MR} tasks\\
ii) IDE event logs can help predict code complexity
}




\noindent\subsection{\textbf{RQ5. Does the development strategy has an influence on teams' development process?.}}

Automatic
IV - NIST\\
DV - PCC\\
DV - KS Is normal, SW Is normal\\
ANOVA - There are differences\\

Manual
Manual
IV - NIST\\
DV - PCC\\
DV - KS Is normal, SW not normal\\
KW - There are no differences\\


Removing Outliers\\
Automatic
IV - NIST\\
DV - PCC\\
DV - KS Is normal, SW Is normal\\
ANOVA - There are differences\\

Manual
IV - NIST\\
DV - PCC\\
DV - KS Is normal, SW Is normal\\
ANOVA - There are no differences\\




\noteboard{RQ5. Summary}{
i) A moderate correlation \textbf{(0.43)} was found between \textbf{VG} and \textbf{PCC} on \textbf{MR} tasks\\
ii) IDE event logs can help predict code complexity
}


\noindent\subsection{\textbf{RQ5. Does the development strategy has an influence on teams' development process?.}}


\subsubsection{Predicting Software Complexity Reduction}
\label{sec:predicting-software-complexity}


\noteboard{RQ5. Summary}{
i) Cluster A\\
ii) Cluster B
}




\noindent\subsection{\textbf{RQ6. Can we profile teams according to their work patterns and productivity levels ?.}}

Event data is usually mined in three perspectives: \textbf{Temporal Proximity}, \textbf{Frequency} and \textbf{Spatial Proximity} \cite{Fukui2019ClusterAnalysis}.

\textbf{Temporal Proximity.} It refers to the occurrence of a set of events within a common temporal window.

\textbf{Frequency.} Addresses the possibility of clustering subjects according to the number of occurrences on one or a set of features.

\textbf{Spatial Proximity.} Introduce the assessment for a certain cluster \textbf{A}, which may exist based in the close proximity within the feature space.








\subsubsection{Detecting Optimal Clusters}
\label{sec:cluster-detection}

\textbf{Step 1: Generating candidate patterns.} First, we generate candidate clusters using hierarchical clustering in the data space without using the time information. All possible pairs of clusters are made into a candidate pattern set after excluding the inclusion relations

\textbf{Step 2: Evaluating candidate patterns.} Next, an evaluation value for each candidate pattern is calculated according to the function L (eq. (5)). When the candidate pattern is greater than or equal to the pre-defined minimum thresholds Lmin and Suppmin, the pattern is added to the output pattern set P

\textbf{Step 3: Excluding overlapped patterns.} Finally, the overlapping patterns within the output pattern set P are removed and the remaining pattern set is used.

\textbf{Optimal number of clusters.} 

Determining the optimal number of clusters in a data set is a fundamental issue in partitioning clustering, such as k-means clustering. The same applies to topic modelling which requires the user to specify the number of topics \textit{\textbf{k}} to be generated.



Unfortunately, there is no definitive answer to this question. The optimal number of clusters is somehow subjective and depends on the method used for measuring similarities and the parameters used for partitioning.
A simple and popular solution consists of inspecting the dendrogram produced using hierarchical clustering to see if it suggests a particular number of clusters. Unfortunately, this approach is also subjective.

Direct methods: consists of optimizing a criterion, such as the within cluster sums of squares or the average silhouette. The corresponding methods are named elbow and silhouette methods, respectively.


\plot{chapter5-1.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]


\subsubsection{Mining Topics}
\label{sec:mining-topics}


\plot{chapter5-2.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-3.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-4.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-5.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-6.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-7.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-8.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-9.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-10.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-11.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-12.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter7-1.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter7-21.pdf}[Optimal number of topics evaluation][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter7-2.pdf}[A sample of a team work session commands with the correspondent frequencies][12][H][trim=6cm 9cm 4cm 9cm]

\input{topics}

\input{accuracy_matrix}

\input{model_70}

\input{model_74}

\input{model_78}

\input{model_83}

\input{model_94}



\begin{comment}
Eclipse View-Long Method, Eclipse Editor-File Editing, Eclipse View-Long Method, Eclipse Editor-File Editing, Eclipse Editor-File Editing, Edit-Undo,
Eclipse View-Package Explorer, Eclipse View-Long Method, Eclipse Editor-File Close, Eclipse View-Feature Envy, Edit-Undo, Eclipse Editor-File Editing, Eclipse Editor-File Editing, Edit-Undo, Eclipse Editor-File Editing, Eclipse View-Feature Envy, Eclipse Editor-File Editing, Eclipse View-Long Method, Eclipse View-Long Method, Edit-Undo, Eclipse Editor-File Editing, Eclipse Editor-File Editing, Eclipse View-Long Method, Eclipse Editor-File Editing, Eclipse Editor-File Editing, Eclipse View-God Class, Eclipse View-Long Method, Eclipse Editor-File Open
\end{comment}


\subsubsection{Results}


%\plot{chapter4-2.pdf}[Studies score per Year at Stage 4][12]

\noteboard{RQ2. Summary}{
i) Exploratory Case Study is the most frequent empirical study found\\
ii) \\
iii)
}

\subsubsection{Implications}


\subsection{RQ3}

\subsubsection{Results}


%\plot{chapter4-3.pdf}[Studies score per Year at Stage 4][12][H]

\noteboard{RQ3. Summary}{
i) Exploratory Case Study is the most frequent empirical study found\\
ii) \\
iii)
}

\subsubsection{Implications}


\begin{comment}


\plot{chapter4-4.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter4-5.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter4-6.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter4-7.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-1.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-10.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-11.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-12.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-13.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-2.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-3.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-4.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-5.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-6.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-7.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-8.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter5-9.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]

\end{comment}

==> kruskal-wallis.tex <==
\begin{table}[H]
\caption{One-Way Kruskal-Wallis Results}
\label{table:kw}
%\centering
\begin{tabular}{clccc}
	\hline\noalign{\smallskip}
		\textbf{Task} & \textbf{Factor} & \textbf{Df.} & \textbf{Chi-Sq.} & \textbf{\textit{Sig.}}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
	%\multicolumn{8}{l}{\textbf{Automatic Refactoring}}\\[0.1cm]
     \textbf{\multirow{2}{*}{\shortstack[c]{Automatic\\ Refactoring}}} & \textbf{IV} & 2 & 288 & \textbf{0.0312*}\\[0.05cm]
    & \textbf{Residuals} &  & 288 & \textbf{0.0312*}\\\\[0.05cm] 
     
      \textbf{\multirow{2}{*}{\shortstack[c]{Manual\\ Refactoring}}} & \textbf{IV} & 2 & 288 & \textbf{0.0312*}\\[0.05cm]
      & \textbf{Residuals} &  & 288 & \textbf{0.0312*}\\[0.02cm] 
     
     
     \noalign{\smallskip}\hline
   \multicolumn{5}{l}{\textit{*Statistically significant if Sig. $<$ 0.05}}\\
   \multicolumn{5}{l}{\shortstack[l]{\textbf{Df.} - Degrees of freedom, \textbf{Chi-Sq.} - Chi-Square,\\ \textbf{Sig.} - Asymptotic Significance (2-tailed)}}
\end{tabular}
\end{table}

==> lda-sdpm.tex <==
\begin{table}[H]
\caption{Traditional Text Mining vs. Software Development Process Mining}
\label{table:sdpm-topic-modelling}
%\centering
\begin{tabular}{llll}
	\hline\noalign{\smallskip}
			\textbf{} & \textbf{TM} & \textbf{SDPM} & \textbf{}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
	%\multicolumn{8}{l}{\textbf{Automatic Refactoring}}\\[0.1cm]
	
	\multicolumn{4}{l}{\cellcolor{gray!10}\textbf{Inputs}}\\[0.1cm]
	\textbf{Corpus} & Documents/Articles & Development Work Sessions & \\[0.1cm]
	\textbf{Document} & Mixture of Topics & Mixture of Behaviours & \\[0.1cm]
	\textbf{Topic} & Frequent Words/Terms & Frequent Actions/Commands & \\[0.2cm]
    % \input{chapter7-topics_latex}
    \multicolumn{4}{l}{\cellcolor{gray!10}\textbf{Outputs}}\\[0.1cm]
	\textbf{Discovers} & Distinct Subjects/Topics & Individuals/Teams Development Patterns & \\[0.1cm]
	\textbf{Usefulness} & Identify Social Trends & Optimize Resource Allocation & \\
	\textbf{} & Frame Research Interests & Detect Practices Deviations & \\
	\textbf{} & Sentiment Analysis & Forensic Project Analysis & \\[0.2cm]
	
   \noalign{\smallskip}\hline
   \multicolumn{4}{l}{\textbf{TM}-Text Mining, \textbf{SDPM}-Software Development Process Mining}\\
   %\multicolumn{4}{l}{\shortstack[l]{\textbf{Df.} - Degrees of freedom, \textbf{Chi-Sq.} - Chi-Square,\\ \textbf{Sig.} - Asymptotic Significance (2-tailed)}}
\end{tabular}
\end{table}

==> ml_metrics.tex <==
 Several metrics are employed in machine learning classification problems for the assessment of
models’ performance. The list bellow serves as a brief introduction to those metrics and how they
are calculated.\\




\noindent\textbf{True Positive (TP).} The outcome prediction was positive, and so was the actual value (e.g., the booking was predicted as likely to cancel and has been effectively canceled).\\
%We computed \textbf{True Positive (TP)} follows: 
%\begin{equation}
%\label{equ:TP}
%\shortstack[l]{\textbf{TP}} =   
%\end{equation}


\noindent\textbf{False Positive (FP).} The outcome prediction was positive, but the actual value was negative (e.g., refactoring was predicted as likely to be automatic, but it was indeed not automatic(manual)). \textbf{Type I error.}\\
%We computed \textbf{False Positive (FP)} as follows: 
%\begin{equation}
%\label{equ:FP}
%\shortstack[l]{\textbf{FP}} =  
%\end{equation}


\noindent\textbf{True Negative (TN).} The outcome prediction was negative, and so was the actual value (e.g., the booking was predicted as likely not to cancel and has been effectively not canceled).\\
%We computed \textbf{True Negative (TN)} follows: 
%\begin{equation}
%\label{equ:TN}
%\shortstack[l]{\textbf{TN}} = 
%\end{equation}


\noindent\textbf{False Negative (FN).} The outcome prediction was negative, but the actual value was positive (e.g., refactoring was predicted as likely not to be automatic(manual), but it was indeed automatic). \textbf{Type II error.}\\
%We computed \textbf{False Negative (FN)} as follows: 
%\begin{equation}
%\label{equ:FN}
%\shortstack[l]{\textbf{FN}} =  
%\end{equation}


\noindent\textbf{Area Under the Curve (AUC).} Measure of success calculated from the area under the plot of true positive rate (TPR) against false positive rate (FPR).\\
%We computed \textbf{Area Under the Curve (AUC)} as follows: 
%\begin{equation}
%\label{equ:AUC}
%\shortstack[l]{\textbf{AUC}} =  
%\end{equation}




\noindent\textbf{Accuracy}. Measure of outcome correctness. Measures the proportion of true results among the total number of predictions and is defined as follows: 
\begin{equation}
\label{equ:Accuracy}
\shortstack[l]{\textbf{Accuracy}} = \frac{\sum{TP} + \sum{TN}}{\sum{TP} +\sum{TN} + \sum{FP} +\sum{FN}} 
\end{equation}\\


\noindent\textbf{False Positive Rate (FPR or Fall-out).} Measures the probability of a positive prediction result
and the actual value being negative (e.g., probability of a refactoring being predicted as likely to be
automatic and effectively it was not). It is defined as follows: 
\begin{equation}
\label{equ:FPR}
\shortstack[l]{\textbf{FPR}} =  \frac{\sum FP}{ \sum FP + \sum TN} 
\end{equation}\\


\noindent\textbf{Precision (Pre.).} Measures the proportion of correct positive predictions. It is defined as follows: 
\begin{equation}
\label{equ:Precision}
\shortstack[l]{\textbf{Precision}} =  \frac{\sum TP}{\sum TP + \sum FP}
\end{equation}\\


\noindent\textbf{True Negative Rate (TNR or Specificity).} Measures the probability of a negative prediction result and the actual value being negative (e.g., probability of a refactoring being identified as not automatic and effectively it was not). It is defined as follows: 
\begin{equation}
\label{equ:TNR}
\shortstack[l]{\textbf{TNR}} =  \frac{\sum TN}{ \sum TN + \sum FP} 
\end{equation}\\



\noindent\textbf{True Positive Rate (TPR, Recall or Sensitivity).} Measures the probability of a positive prediction result and the actual value being positive (e.g., probability of a refactoring being identified as likely to be automatic and effectively was automatic). It is defined as follows: 
\begin{equation}
\label{equ:TPR}
\shortstack[l]{\textbf{TPR}} =  \frac{\sum TP}{ \sum TP + \sum FN}
\end{equation}\\


\noindent\textbf{F1 Score.} Is the harmonic mean of precision and sensitivity. It is defined as follows: 
\begin{equation}
\label{equ:F1}
\shortstack[l]{\textbf{F1}} = 2 * \frac{Precision * Recall}{Precision + Recall} 
\end{equation}\\

\begin{equation}
\label{equ:F2}
\shortstack[l]{\textbf{F1}} = 2 * \frac{  \frac{\sum TP}{\sum TP + \sum FP}  * \frac{\sum TP}{ \sum TP + \sum FN} }{  \frac{\sum TP}{\sum TP + \sum FP}  + \frac{\sum TP}{ \sum TP + \sum FN}} 
\end{equation}




==> normality.tex <==

\begin{table}[H]
\caption{Normality Tests}
\label{table:normality-test}
%\centering
\begin{tabular}{p{1.5cm}cccp{0.01cm}ccc}
	\hline\noalign{\smallskip}
	& \multicolumn{3}{c}{\cellcolor{gray!10}\textbf{Kolmogorov-Smirnov}} & & \multicolumn{3}{c}{\cellcolor{gray!10}\textbf{Shapiro-Wilk}}\\
	\textbf{Factor} & \textbf{\textit{Statistics(D)}} & \textbf{\textit{df}} & \textbf{\textit{Sig.}} & &
	\textbf{\textit{Statistics(W)}} & \textbf{\textit{df}} & \textbf{\textit{Sig.}}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

    \textbf{PRODIDX} & 0.349 & 5 & 0.045 & & 0.768 & 5 & \textbf{0.043*} \\[0.1cm]
    \textbf{VG} & 0.349 & 5 & 0.045 & & 0.768 & 5 & \textbf{0.043*} \\[0.1cm]
    \textbf{PCC} & 0.349 & 5 & \textbf{0.045*} & & 0.768 & 5 & 0.043 \\[0.05cm] 
 %\input{correlation_man_body}

   \noalign{\smallskip}\hline
   	\multicolumn{3}{l}{\textit{*Statistically significant if Sig. $<$ 0.05}}
\end{tabular}
\end{table}

==> pol.tex <==


\subsection{Software Development and the \texorpdfstring{\textit{$"$Pollock Effect$"$}}{}} % (fold)
\label{sec:intro-pollock-effect}
The \textbf{XX} century have seen the birth of one of the most talented painters and a major figure in the abstract expressionist movement, Jackson Pollock.
Despite many controversy around his lifestyle, he was admired by his innovative painting technique. It consisted of pouring or splashing liquid household paint onto a horizontal surface (‘drip technique’), enabling him to view and paint his canvases from all angles.
The final work would be the culminate of multiple layers of paint on top of each other, resulting from multiple sessions of creative work, which, only when combined produced the overwhelming visual effects we found in Pollocks' art \cite{JacksonPollock,JacksonStyle}.

During many years, art critics, historians and admirers have looked at Pollocks' art only as the result of his geniality from the creative perspective.
Nowadays, researchers, mainly physicists, argue that his work is not just the product of a creative session, it is also supported by a few laws of physics \cite{Herczynski2011PaintingSheets}. Many are convinced that these laws are able to capture the author fingerprints and authenticity, thus allowing to distinguish a genuine Pollock painting from a similar product created by another artist that was inspired by Pollocks' method.

Despite the fact that his technique was disruptive, one thing remains the same, the painting is the final product. However, the means by which he achieved it have one fundamental difference from other painting styles. The workspace conditions were different: canvas on the floor, ability to paint from multiple perspectives, using different materials and objects, exploring fluid dynamics and finally, letting gravity perform the final touch.

Jackson Pollock, unconsciously, created not only a new painting technique which produces innovative visually impactful products, he authored a new painting process.

The software development ecosystem have some similarities with Pollocks' framework. It consists of many overlaid sessions of work of one or many developers, having a multitude of workspace conditions, looking and interacting with it from multiple angles, and yet contributing to a unified software product build. These work sessions overlap in time and when one looks at them globally and from different perspectives many insights come to the daylight. Several aspects, which initially seems like the result of a creative process, may very well be the outcome of a few laws science may explain and contain implicit behaviors with an impact on the final product we are yet to fully comprehend. The more data we have and from more data sources covering all the process facets the better we can analyze and explain a software development process. However, sometimes its not possible or easy to get data from distinct data sources in order to conduct research studies. That's where the IDE may bring additional value, as it is probably the tool that can provide more information to analyze parts of or a complete software development process.


\begin{comment}
Jackson Pollock, unconsciously, created not only a new painting technique which inspired many artists\footnote{In Figure \ref{fig:pollock} (right), Adam Zafrian art inspired by Pollocks' painting process - \href{https://bit.ly/35aivrK}{https://bit.ly/35aivrK}}
 after him, he forged/authored a new painting process\footnote{In Figure \ref{fig:pollock} (left), Jackson Pollock at work in 1949, photographed by Martha Holmes. Pollock appears to be using a relatively viscous paint that forms a continuous jet of fluid he controls by moving a trowel up, down, or across the canvas. (Photograph @ Time, Inc, Getty Images) - Adapted from \cite{Herczynski2011PaintingSheets}.}

\graphic{ht!}{pollock3.png}{Pollock Process/Painting}{14}{fig:pollock}
\end{comment}



\begin{comment}
As recalled by Maurice Wilkes,1 speaking of his programming experiences
from the early 1950s: “It was on one of my journeys between the
EDSAC room and the punching equipment that ‘hesitating at the
angles of stairs’ the realization came over me with full force that a
good part of the remainder of my life was going to be spent in finding
errors in my own programs.”
\end{comment}


==> preliminaries.tex <==

\begin{comment}

\textbf{Feature Extraction.} This step encodes every single trace of the input event logoff each of the two process variants, into a set of vectors of the same length for every event. Each vector contains the respective wavelet coefficients for a specific event. Essentially, a wavelet coefficient is an encoding of the time series behind each  trace.  For  a  trace,  these  vectors  are  stacked  into  a  single  vector.  This  way allows the encoding of a process variant as a matrix, called design matrix, which is used in the next step 



\textbf{Feature Selection.} n this step, the wavelet coefficients are used to build features to train a binary classifier. This procedure can be repeated several times for cross-validation purposes, and a statistical test is performed on top of the results of cross-validation, to ensure that the selected features (events classes in the log) provide enough information to discriminate the two classes arising from the two process variants. 


\textbf{Filtering.} This  last  step  filters  the  log  of  each  process  variant  by  keeping  only those traces that contain discriminatory events discovered from the previous stage.A mutual fingerprint is then built from the traces left for each process variant log 


\subsection{Preliminaries}

In  this  section  we  introduce  preliminary  definitions  required  to  describe  our  approach such as event, trace, event log and process variant. Next, we provide some basic linear algebra definitions that will be specifically used for our featuring encoding.


\noindent\textbf{Definition 1 (Event, Trace, Event Log)}. 
\begin{itemize}
    \item \textit{ An event can be defined as a tuple (a, c, t, $\{$(p\textsubscript{1},v\textsubscript{1}),...,(p\textsubscript{n},v\textsubscript{n})$\}$) where a is the process activity name, c is the case id, t is the timestamp and set $\{$(p\textsubscript{1},v\textsubscript{1}),...,(p\textsubscript{n},v\textsubscript{n})$\}$ (where n $\geqslant0$) are the event or case properties/attributes and their values.}
    \item \textit{A trace is a non-empty sequence $\sigma$=$\{$e\textsubscript{1},...,e\textsubscript{n}$\}$ of events such that $\forall$i,j $\in$ [1..n] e\textsubscript{i}.c=e\textsubscript{j}.c.} 
    \item \textit{An event log is a set of traces and can be defined as L=$\{$$\sigma$\textsubscript{1},...,$\sigma$\textsubscript{n}$\}$}.\\
\end{itemize}


\noindent\textbf{Definition 2 (Process variant)}. 
\begin{itemize}
   \item \textit{An event log L can be partitioned into a finite set of groups called process variants $\varsigma$\textsubscript{1},$\varsigma$\textsubscript{2},...,$\varsigma$\textsubscript{n}, such that $\exists$p such that $\forall$ $\varsigma$\textsubscript{k} and $\forall$ $\sigma$\textsubscript{i},$\sigma$\textsubscript{j} $\in$ $\varsigma$\textsubscript{k}, $\sigma$\textsubscript{i}.p=$\sigma$\textsubscript{j}.p.}
\end{itemize}


\indent The  above  definition  of  a  process  variant  emphasizes  that  process  executions in the same group must have the same value for a given attribute, and each process execution belongs only to one process variant.\\


\noindent\textbf{Definition 3 (Vector).} 
\begin{itemize}
    \item \textit{A vector, X=(x\textsubscript{1},x\textsubscript{2},...,x\textsubscript{n})\textsuperscript{T}, is a column array of elements where the ith element is shown by x\textsubscript{i}. If each element is in $\mathbb{R}$ and vector contains n elements, then the vector lies in $\mathbb{R}$\textsuperscript{n×1}, and the dimension of X, dim(X), is n×1.}\\
   
\end{itemize}

  We represent a set of d vectors as X\textsuperscript{(1)},X\textsuperscript{(2)},...,\textsuperscript{(d)}, where X\textsuperscript{i} $\in$ $\mathbb{R}$\textsuperscript{n×1}. Also, they can be represented by a matrix M=(X\textsuperscript{(1)},X\textsuperscript{(2)},...,X\textsuperscript{(d)}) where M $\in$ $\mathbb{R}$\textsuperscript{n×d}. We denote  the ith row of a matrix by M\textsubscript{i,:}, and like wise the i th column by M\textsubscript{:,i}. The previous definitions can be extended for a set of columns or rows, for example if R={3,5,9} and C={1,4,6,12}, then M\textsubscript{R,C} returns the indicated rows and columns.\\


\noindent \textbf{Definition 4 (Vector space).} 
\begin{itemize}
\item \textit{A vector space consists of a set V of vectors, a field $\mathbb{F}$ ($\mathbb{R}$ for real numbers), and two operations +,× with the following properties, $\forall$u, v $\in$ V, u+v $\in$ V, and $\forall$c $\in$ F, $\forall$v $\in$V, c×v $\in$V.}
\end{itemize}


\end{comment}


\begin{comment}

In the context of process, methodologies and productivity, existing concepts need to be redefined for meeting the
current needs of the industry. Software process is a well-investigated research area, but nowadays there are several
new advancements in technology and practice that introduce significant changes in this aspect. A new notion of
productivity should be defined, where “lines of code” is not anymore the right measure of productivity, but software
is measured in terms of its other qualities, usability, reliability, scalability. New possibilities to easily gather user
feedback and monitoring information have the potential to enable an informed evolution of software while shorter
development cycles call for novel software production methodologies to actually enable controlled management of
such short development cycles. 

\end{comment}



==> pseudo-code.tex <==
%\begin{comment}

%\noteboard{RQ4. Summary}{
%i) A moderate correlation \textbf{(0.43)} was found between \textbf{VG} and \textbf{PCC} on \textbf{MR} tasks\\
%ii) IDE event logs can help predict code complexity
%}

%\subsubsection{Implications}


\begin{algorithm}[H]
\SetAlgoLined
%\SetAlgoNoLine
\KwIn{Event Log}
\KwResult{Process Metrics Matrix}
 initialization\;
 
 \While{While condition}{
  instructions\;
  \eIf{condition}{
   instructions1\;
   instructions2\;
   }{
   instructions3\;
  }
  
  %\lForEach{element $e$ of the line $i$}{\FindCompress{p}}
  
    \For{$i\leftarrow 2$ \KwTo $l$}{
    }
    
}
  

\caption{How to write algorithms}
\end{algorithm}

%\newcommand{\forcond}{$i=0$ \KwTo $n$}
\SetKwFunction{FRecurs}{FnRecursive}%



\begin{algorithm}[H]
\SetAlgoLined
%\SetAlgoNoLine

 
 %\SetKwFunction{FMain}{NegationDetection}
 %\SetKwFunction{FMain}{NegationDetection}
    \SetKwProg{Fn}{Function}{:}{}
 %   \Fn{\FMain{$F$}}{
    
 %   }
 \Fn(\tcc*[h]{recursive algorithm}){\FRecurs{some args}}{ 
  
\KwIn{Event Log}
\KwResult{Process Metrics Matrix}
initialization\;
 
  \For{$i\leftarrow 2$ \KwTo $l$}{
     }
 
 }
 
\textbf{End Function}
\caption{How to write a function algorithms}
\end{algorithm}

%\end{comment}



==> statements.tex <==
 
Studies are being done where practitioners can see, not where there are things to find \cite{2016PerspectivesEngineering}.

The decision making process is the most important part of analytics \cite{2016PerspectivesEngineering}.


Finally, using a combination of regression modeling, text analysis, and visualization, we examined the interactions of language, language properties, application domain and defect type.


Relevant studies have been performed to examine the impact of languages in the software quality.  As opposed to common belief, in general, language choice does not impact software quality much \cite{2016PerspectivesEngineering}.


Code Review is expensive. Modern code reviewing traces back its roots to the process of inspection \cite{2016PerspectivesEngineering}.
 
IDE data is just sitting still, waiting to provide insights. It is suffering from the Parkinson's law of triviality, where practitioners, rather than exploring the data, spend time discussing minor details. This phenomena, is also related to "analysis paralysis", where transitioning from discussing something to actually doing it it is overwhelming and inhibits progress.


Causal relationship is formed based on two processes in which one of them (cause) is partly responsible for the occurence or change of the other (effect).
The direction of causal relationships is not two-sided as in correlations.


Not everything is recorded in sofwtare repositories.
Software repositories contain noisy data, such as misclassification of artifacts(eg: issue reports classified as bug fixes when they are related with new features)

Innacurate categorization of bugs, where 40\% ar believed to be wrong.

Version control systems are not granular enough
Commits are snapshots in time.


When a file/class is found to be the cause of many bugs, its not only enough to check version control systems, as they are not granular enough. It is imperative to understand who touched that artifact, when, for how long and how much of that time was really spent executing coding activities on it. It is important to go backwards and gather evidences of how the artifact was build, and not simply how was it at the moment of check-in. it is vital to understand the developer behavior and effective actions, iddle time and possible transitions to other activities which may defocus the individual from what he was supposed to perform.
Its about the efficiency and effectiveness of developers under normal and stressful situations that matters to study.


Reports show that organizations are finding bugs in just 10\% of the code.

An actionable software development metric is one that measures a property directly under a developers' control. An emergent metric is one that aggregates a variety of potential problems into a single measurement without an obvious diagnosis.
Actionable metrics tells us how to improve. Emergent metrics tells us where we are.



Traditional SPI trieds to define processes in order to optimize them. However, it is often challenging to distinguish between officla defined processes and actual processes used in practice. An alternative is to deduce the software processes from the data gathered from actual software development, resulting in a description of the actual process, not just the official or desired process. This data can also be sued to analyze the workflows and identify bottlenecks.


Hopefully we could make little contributions to change how researchers think about and approach the mining of development processes, as well as how developers think about their individual work. 
It was a combination of painstaking work, subtle insights , unique perspectives and sometimes just luck. It is not necessarily repeatable, it cannot be forced, and at least some parts of it cannot be taught. \cite{2016PerspectivesEngineering}.

Some years ago, the Dagsthul Seminar on Software Development Analytics took place for the first time. That venue produced some of the most remarkable notes, guidelines and recommendations for the software engineering community. On that event, many data sources were identified as being at our disposal for sotfware develoment analytics purposes. However, many of those sources were not, and are to today, not being mined with enough emphasis and sufficient attention from practitioners.



Sjober and Dyba
A therory should represent knowledge that is somewhat widely applicable but still not trivial, or one that follows from a definition. In disciplines that involve human behavior, one would hardly find such universal theories.
It is though a challenge to define an appropriate scope for a SE theory.

Paraphrasing Bunge - premature theorizing is likelly to be wrong- but not sterile- and that a long deferred beginning of theorizing is worse that any number of failures.
the relevant 



There will be a fundamental shift in the software engineering domain, particularly in the software development analytics space. The mining of activities performed by developers, testers and many other individuals involved in a software project will complement any code related analysis. It will be present in any product and project management activities from day zero. Sooner or later, this practice will provide fully validated evidences needed to understand, from a different perspective, why certain pieces of software fail more than others. More important, it may bring deeper insights on what were the events, decisions and actions taken which have contributed most for any undesired outcomes as well as the actors involved.



==> teams-productivity.tex <==


\begin{table}[H]
\caption{Teams' Productivity Results}
\label{table:teams-productivity}
\centering
\begin{tabular}{clcccccc}
	\hline\noalign{\smallskip}
	\textbf{\#} & \textbf{Metric Name} & \textbf{Min.} & \textbf{1st Qu.} & \textbf{Median} & \textbf{Mean} & \textbf{3rd Qu.} &\textbf{Max.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
	\multicolumn{8}{l}{\textbf{Automatic Refactoring}}\\[0.2cm]
     \textbf{1} & \textbf{PRODIDX} & 2.68\% & 5.87\% & 6.95\% & 7.81\% & 8.84\% & 16.77\%\\[0.2cm]
    & & \multicolumn{6}{c}{\textbf{Outliers: Lower $<$ -0.051\% ; Upper $>$ 0.1686\%}}\\[0.5cm]
     \multicolumn{8}{l}{\textbf{Manual Refactoring}}\\[0.2cm]
     \textbf{2} & \textbf{PRODIDX} & 0.32\%  &  0.62\% &   0.94\% &   2.69\%  &  3.92\%  & 13.98\%\\[0.2cm]
     & & \multicolumn{6}{c}{\textbf{Outliers: Lower $<$ -0.0104\% ; Upper $>$ 0.0254\%}}\\[0.2cm]
     \noalign{\smallskip}\hline\\
   \multicolumn{8}{l}{\shortstack[c]{\textbf{PRODIDX} - As computed in Equation \ref{equ:Productivity}}}
\end{tabular}
\end{table}



==> tools.tex <==
\begin{table}[H]
\caption{Software Tools Used}
\label{table:software-tools}
%\centering
\begin{tabular}{llll}
	\hline\noalign{\smallskip}
	%& \multicolumn{3}{c}{\cellcolor{gray!10}\textbf{Kolmogorov-Smirnov}} & & \multicolumn{3}{c}{\cellcolor{gray!10}\textbf{Shapiro-Wilk}}\\
	\textbf{Software} & \textbf{Usage/Purpose} & \textbf{URL} & \textbf{Obs.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
	
	\multicolumn{4}{l}{\cellcolor{gray!10}\textbf{Software Development}}\\[0.1cm]
    \textbf{Eclipse} & Software Development Process Mining Plugin & \href[pdfnewwindow=true]{ https://www.eclipse.org/}{ https://www.eclipse.org/} & \\[0.1cm]
    \textbf{Sublime Text} & Engine for Event Standardization, & \href[pdfnewwindow=true]{ https://www.sublimetext.com/}{ https://www.sublimetext.com/} & \\[0.1cm]
    & Formatting and Aggregation &  & \\[0.3cm]
   
   
    \multicolumn{4}{l}{\cellcolor{gray!10}\textbf{Event Persistence Layer}}\\[0.1cm]
    \textbf{CSV Files} & Store Events Locally at Runtime & & \\[0.1cm]
    \textbf{Kafka} &  Store Events Locally or Remotely at Runtime & \href[pdfnewwindow=true]{ https://kafka.apache.org/}{ https://kafka.apache.org/} & \\[0.1cm]
    \textbf{Azure EventHub} & Store Events Locally or Remotely at Runtime & \href[pdfnewwindow=true]{ https://azure.microsoft.com/en-in/services/event-hubs/}{ https://azure.microsoft.com/en-in/services/event-hubs/} & \\[0.1cm]
    \textbf{Trello Rest API} & Load Software Project Tasks at Runtime & \href[pdfnewwindow=true]{ https://developer.atlassian.com/cloud/trello/rest/}{ https://developer.atlassian.com/cloud/trello/rest/} & \\[0.3cm]
   
    \multicolumn{4}{l}{\cellcolor{gray!10}\textbf{Event Repository, Transformation and Exporting}} \\[0.1cm]
    \textbf{MySQL} & Store, transform and query events & \href[pdfnewwindow=true]{https://www.mysql.com/}{ https://www.mysql.com/} &  \\[0.1cm]
     & to generate process metrics &  &  \\[0.3cm]
   
   \multicolumn{4}{l}{\cellcolor{gray!10}\textbf{Process Mining}}\\[0.1cm]
   \textbf{Prom} & Process Discovery and Conformance Checking & \href[pdfnewwindow=true]{ http://www.promtools.org/}{ http://www.promtools.org/} &  \\[0.1cm]
   \textbf{StateChart Workbench} & Process Complexity Metrics Extraction & & \\[0.3cm]
 
   \multicolumn{4}{l}{\cellcolor{gray!10}\textbf{Product Metrics}}\\[0.1cm]
   \textbf{Metrics} & Software Metrics Extraction & \href[pdfnewwindow=true]{ http://metrics.sourceforge.net/ }{ http://metrics.sourceforge.net/ } &  \\[0.3cm]
   
   \multicolumn{4}{l}{\cellcolor{gray!10}\textbf{Statistical Analysis}}\\[0.1cm]
   \textbf{R} & Data Transformation, charts generation and export & \href[pdfnewwindow=true]{ https://www.r-project.org/}{ https://www.r-project.org/} &  \\[0.1cm]
   \textbf{R Studio} & Main Data Science Workbench & \href[pdfnewwindow=true]{ https://rstudio.com/}{ https://rstudio.com/} & \\[0.3cm]
 
   \multicolumn{4}{l}{\cellcolor{gray!10}\textbf{Machine Learning Algorithms}}\\[0.1cm]
   \textbf{Weka} & Model Selection and Hyperparameter Optimization & \href[pdfnewwindow=true]{ https://www.cs.waikato.ac.nz/ml/weka/}{ https://www.cs.waikato.ac.nz/ml/weka/} & \\[0.3cm]
  
   \multicolumn{4}{l}{\cellcolor{gray!10}\textbf{Thesis Writing}}\\[0.1cm]
   \textbf{Draw.io} & Diagram Management & \href[pdfnewwindow=true]{ https://www.draw.io/}{ https://www.draw.io/} &  \\[0.1cm]
   \textbf{Mendeley} & Reference Management & \href[pdfnewwindow=true]{ https://www.mendeley.com/}{ https://www.mendeley.com/} &  \\[0.1cm]
   \textbf{Overleaf} & Document Management & \href[pdfnewwindow=true]{ https://www.overleaf.com/}{ https://www.overleaf.com/} &  \\[0.1cm]
 
   \noalign{\smallskip}\hline
   %\multicolumn{3}{l}{\textit{*Statistically significant if Sig. $<$ 0.05}}
\end{tabular}
\end{table}

==> topics-patterns.tex <==

\begin{table}[H]
\caption{Top 15 Teams by VG reduction}
\label{table:topics-patterns}
%\centering
\begin{tabular}{ccccc}
	\hline\noalign{\smallskip}
	%& \multicolumn{2}{c}{\cellcolor{gray!10}\textbf{VG}}\\
	\textbf{Team} & \textbf{Grade} &  \textbf{PCC} & \textbf{VG} & \textbf{Refactoring Pattern}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

 \input{chapter7-ComplianceDataset}

   \noalign{\smallskip}\hline
   	%\multicolumn{3}{l}{\textit{*Statistically significant if p-value $<$ 0.05}}
\end{tabular}
\end{table}

==> topics.tex <==
\begin{table}[H]
\caption{Topics}
\label{table:topics}
%\centering
\begin{tabular}{cllc}
	\hline\noalign{\smallskip}
		\textbf{Topic} & \textbf{Activity Type} & \textbf{Term} & \textbf{Beta}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
	%\multicolumn{8}{l}{\textbf{Automatic Refactoring}}\\[0.1cm]
     
     \input{chapter7-topics_latex}
     
   \noalign{\smallskip}\hline
   %\multicolumn{4}{l}{\textit{*Statistically significant if Sig. $<$ 0.05}}\\
   %\multicolumn{4}{l}{\shortstack[l]{\textbf{Df.} - Degrees of freedom, \textbf{Chi-Sq.} - Chi-Square,\\ \textbf{Sig.} - Asymptotic Significance (2-tailed)}}
\end{tabular}
\end{table}

==> variables.tex <==

\begin{table}[H]
\caption{Variable Details}
\label{table:variable-details}
%\centering
\begin{tabular}{lcl}
	\hline\noalign{\smallskip}
	\textbf{Factor} & \textbf{Admissible Values} & \textbf{Description}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
    %\multirow{}{}{}
    \multirow{4}{*}{\textbf{PCC\_LEVEL}} & \textbf{LOW} & \multirow{4}{*}{Just a description which can be long}\\[0.1cm]
    & \textbf{MEDIUM} & \\[0.1cm]
    & \textbf{HIGH} & \\[0.1cm]
    & \textbf{VERY HIGH} & \\[0.1cm]
  
   \noalign{\smallskip}\hline
   %\multicolumn{3}{l}{\shortstack[l]{\textbf{DF} - Degrees of freedom}}\\
   %\multicolumn{3}{l}{\textit{*Statistically significant if Sig. $<$ 0.05}}
\end{tabular}
\end{table}

==> variance.tex <==

\begin{table}[H]
\caption{Teams' Productivity Results}
\label{table:teams-productivity}
\centering
\begin{tabular}{clcccccc}
	\hline\noalign{\smallskip}
	\textbf{\#} & \textbf{IV} & \textbf{DV} & \textbf{KS Test} & \textbf{SW Test} & \textbf{Variance Test} & \textbf{Results} &\textbf{Max.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
	%\multicolumn{8}{l}{\textbf{Automatic Refactoring}}\\[0.2cm]
     \textbf{AR} & \textbf{PCC\_LEVEL} & \textbf{PRODIDX} & 5.87\% & 6.95\% & 7.81\% & 8.84\% & 16.77\%\\[0.2cm]
    %& & \multicolumn{6}{c}{\textbf{Outliers: Lower $<$ -0.051\% ; Upper $>$ 0.1686\%}}\\[0.5cm]
     %\multicolumn{8}{l}{\textbf{Manual Refactoring}}\\[0.2cm]
     \textbf{MR} & \textbf{PCC\_LEVE}L & \textbf{PRODIDX} &  0.62\% &   0.94\% &   2.69\%  &  3.92\%  & 13.98\%\\[0.2cm]
     %& & \multicolumn{6}{c}{\textbf{Outliers: Lower $<$ -0.0104\% ; Upper $>$ 0.0254\%}}\\[0.2cm]
     \noalign{\smallskip}\hline\\
   \multicolumn{8}{l}{\shortstack[c]{\textbf{PRODIDX} - As computed in Equation \ref{equ:Productivity}}}
\end{tabular}
\end{table}

